Imaging of buried objects from multi-frequency experimental data using a globally convergent inversion method

This paper is concerned with the numerical solution to a 3D coefficient inverse problem for buried objects with multi-frequency experimental data. The measured data, which are associated with a single direction of an incident plane wave, are backscatter data for targets buried in a sandbox. These raw scattering data were collected using a microwave scattering facility at the University of North Carolina at Charlotte. We develop a data preprocessing procedure and exploit a newly developed globally convergent inversion method for solving the inverse problem with these preprocessed data. It is shown that dielectric constants of the buried targets as well as their locations are reconstructed with a very good accuracy. We also prove a new analytical result which rigorously justifies an important step of the so-called "data propagation" procedure.

==> mathmacros.tex <==
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\renewcommand{\phi}{\varphi}
\renewcommand{\d}{\mathrm{d}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ol}{\overline}
\renewcommand{\i}{\mathrm{i}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\mur}{\mu_{\mathrm{r}}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\per}{\mathrm{per}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\smooth}{\text{sm}}
\newcommand{\RR}{R}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\sc}{\mathrm{sc}}
\newcommand{\inc}{\mathrm{inc}}


\DeclareMathOperator{\sign}{\mathrm{sign}}
\DeclareMathOperator{\Id}{\mathrm{Id}}


 \newtheorem{remark}[theorem]{Remark}

\renewcommand{\Re}{\mathrm{Re}\,}
\renewcommand{\Im}{\mathrm{Im}\,}
 \newcommand{\smalf}{\par\smallskip\noindent}
 \newcommand{\medlf}{\par\medskip\noindent}
 \newcommand{\biglf}{\par\bigskip\noindent}

\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsi}{\epsilon}
\newcommand{\oD}{\overline{D}}
\newcommand{\oS}{\overline{S}}
\newcommand{\ov}{\overline}
\newcommand{\pD}{\partial D}
\newcommand{\cO}{{\cal O}}
\newcommand{\bH}{{\bm{H}}}
\newcommand{\vbH}{{\vec{\bm{H}}}}
\newcommand{\bE}{{\bm{E}}}
\newcommand{\vbE}{{\vec{\bm{E}}}}
\newcommand{\vbJ}{{\vec{\bf J}}}
\newcommand{\vbA}{\mathcal{\bm{A}}}
\newcommand{\bD}{{\bm{D}}}
\newcommand{\bRe}{{\bm{\mathcal{R}}^\epsilon}}
\newcommand{\bTe}{{\bm{\mathcal{T}}^\epsilon}}
\newcommand{\vbD}{{\vec{\bm{D}}}}
\newcommand{\curl}{{\vec{\nabla}\times}}
\newcommand{\divv}{{\vec{\nabla}\cdot}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\curll}{\mathrm{curl}}
\newcommand{\divtt}{{\nabla^\bot\cdot}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cR}{{\cal R}}
\newcommand{\pa}{\partial}
\newcommand{\nal}{\nabla_{\alpha}}
\newcommand{\nalT}{\nabla_{\alpha,T}}
\newcommand{\naT}{\nabla_T}
\newcommand{\intO}{\int_{\Omega}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
%\newcommand{\vbz}{\vec{\bm{z}}}
%\newcommand{\vx}{\vbx}
%\newcommand{\bx}{\bm{x}}
%\newcommand{\vbn}{\vec{\bm{n}}}
%\newcommand{\vbut}{\vec{\bm{u}}^t}
%\newcommand{\vbui}{\vec{\bm{u}}^i}
%\newcommand{\vbuis}{\vec{\bm{u}}^{i(s')}}
%\newcommand{\vbu}{\vec{\bm{u}}}
%\newcommand{\vbg}{\vec{\bm{g}}}
%\newcommand{\vbf}{\vec{\bm{f}}}
%\newcommand{\vbw}{\vec{\bm{w}}}
%\newcommand{\vbv}{\vec{\bm{v}}}
%\newcommand{\vbphi}{\vec{\bm{\varphi}}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cm}{{\mathcal M}}
\newcommand{\lin}{\big<}
\newcommand{\rin}{\big>}
\newcommand{\bV}{\boldsymbol{\mathcal{V}}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bd}{{\bf d}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\icu}{{\mbox{\tiny curl}}}
\newcommand{\idiv}{{\mbox{\tiny div}}}

